Degradation Estimation Recurrent Neural Network with Local and Non-Local Priors for Compressive Spectral Imaging

In the Coded Aperture Snapshot Spectral Imaging (CASSI) system, deep unfolding networks (DUNs) have demonstrated excellent performance in recovering 3D hyperspectral images (HSIs) from 2D measurements. However, some noticeable gaps exist between the imaging model used in DUNs and the real CASSI imaging process, such as the sensing error as well as photon and dark current noise, compromising the accuracy of solving the data subproblem and the prior subproblem in DUNs. To address this issue, we propose a Degradation Estimation Network (DEN) to correct the imaging model used in DUNs by simultaneously estimating the sensing error and the noise level, thereby improving the performance of DUNs. Additionally, we propose an efficient Local and Non-local Transformer (LNLT) to solve the prior subproblem, which not only effectively models local and non-local similarities but also reduces the computational cost of the window-based global Multi-head Self-attention (MSA). Furthermore, we transform the DUN into a Recurrent Neural Network (RNN) by sharing parameters of DNNs across stages, which not only allows DNN to be trained more adequately but also significantly reduces the number of parameters. The proposed DERNN-LNLT achieves state-of-the-art (SOTA) performance with fewer parameters on both simulation and real datasets.

==> tables/table4.tex <==
% \begin{table}[!htbp]
%     \centering
%     \scalebox{0.9}{
%         \begin{tabular}{c c c  c c c c}
%             %\small
%             \toprule
%               Model &  LR & BS \\
%             \midrule
%               DERNN-LNLT 3stg & 2 \times $10^{-3}$ & 16 \\
%                 DERNN-LNLT 5stg & 1 \times $10^{-3}$ & 10 \\
%               DERNN-LNLT 7stg & 1 \times $10^{-3}$ & 8 \\
%                 DERNN-LNLT 9stg & 1 \times $10^{-3}$ & 3 \\
%                 DERNN-LNLT 9stg$^*$ & 1 \times $10^{-3}$ & 3 \\
%                 DERNN-LNLT 5stg real & 1 \times $10^{-3}$ & 1 \\
%             \bottomrule
%         \end{tabular}
%     }
%     \caption{\small The learning rate and batch size of different models. }
%     \label{tab:LR and BS}
% \end{table}

\begin{table}[!htbp]
    \centering
    \caption{\small The learning rate and batch size of different models. }
    \begin{tabular}{c c c}
        \toprule
          Model &  LR & BS \\
        \midrule
          DERNN-LNLT 3stg & $2 \times 10^{-3}$ & 16 \\
          DERNN-LNLT 5stg & $1 \times 10^{-3}$ & 10 \\
          DERNN-LNLT 7stg & $1 \times 10^{-3}$ & 8 \\
          DERNN-LNLT 9stg & $1 \times 10^{-3}$ & 3 \\
          DERNN-LNLT 9stg$^*$ & $1 \times 10^{-3}$ & 3 \\
          DERNN-LNLT 5stg real & $1 \times 10^{-3}$ & 1 \\
        \bottomrule
    \end{tabular}
    \label{tab:LR and BS}
\end{table}
